Towards Flexible Time-to-event Modeling: Optimizing Neural Networks via Rank Regression

Time-to-event analysis, also known as survival analysis, aims to predict the time of occurrence of an event, given a set of features. One of the major challenges in this area is dealing with censored data, which can make learning algorithms more complex. Traditional methods such as Cox's proportional hazards model and the accelerated failure time (AFT) model have been popular in this field, but they often require assumptions such as proportional hazards and linearity. In particular, the AFT models often require pre-specified parametric distributional assumptions. To improve predictive performance and alleviate strict assumptions, there have been many deep learning approaches for hazard-based models in recent years. However, representation learning for AFT has not been widely explored in the neural network literature, despite its simplicity and interpretability in comparison to hazard-focused methods. In this work, we introduce the Deep AFT Rank-regression model for Time-to-event prediction (DART). This model uses an objective function based on Gehan's rank statistic, which is efficient and reliable for representation learning. On top of eliminating the requirement to establish a baseline event time distribution, DART retains the advantages of directly predicting event time in standard AFT models. The proposed method is a semiparametric approach to AFT modeling that does not impose any distributional assumptions on the survival time distribution. This also eliminates the need for additional hyperparameters or complex model architectures, unlike existing neural network-based AFT models. Through quantitative analysis on various benchmark datasets, we have shown that DART has significant potential for modeling high-throughput censored time-to-event data.

==> sections/1_introduction_old.tex <==
% 논문에 추가할 것: 
% 좀 더 다양한 생존분석 논문들 (베이스라인에 없더라도, 주요 포인트 언급)
% Loss의 백그라운드 설명 (인디케이터가 필요한 이유 등)
% DATE보다 좋은점 : 단순하고 빠른데 성능 좋다. 
% DATE 장단점: implicit probability distributions을 학습한다는 장점은 있지만, GAN 구조상 mode collapse 가 발생할 수있고 (VEEGAN 논문 참조), 딥러닝 특성상 calibration이 어렵다(deep cox mixture 논문 참조)
% VEEGAN: Reducing Mode Collapse in GANs using Implicit Variational Learning 에서의 설명. "Despite an enormous amount of recent work, GANs are notoriously fickle to train, and it has been observed [1, 19] that they often suffer from mode collapse, in which the generator network learns how to generate samples from a few modes of the data distribution but misses many other modes, even though samples from the missing modes occur throughout the training data."
% DRAFT의 rank-aware loss와 차이점은?
% 
% CoxCC (CoxTime)는 risk set을 subset으로 쪼개서 PH가정 없이도 가능하게끔 만든 모델이라 subset을 얼마나 잘 쪼개는냐에 따라 성능이 갈린다. 대신 training 시간이 굉장히 길어진다. 계산복잡도 살펴보기.
% Right ceonsoring을 가정하지만, interval censoring까지도 확장가능성 내지는 future direction.
% DATE와 DRAFT, DART의 실제 output distribution 비교
% 우리껀 loss function 하나만 쓰는 심플한 형태.
% 생존분석 교과서: kleinbaum2010survival
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Introduction}
% General introduction to time-to-event analysis
Time-to-event analysis, also known as survival or failure time analysis, is a major statistical approach in various fields such as biostatistics, medicine, and economics to estimate either risk scores or the  distribution of event time, given a set of features of subjects  \cite{vigano2000survival,cheng2016computer,dirick2017time,li2021difficulty}.
There are benefits of assessing risk or quantifying survival probabilities but, for all that, time-to-event analysis itself is challenging because of the existence of censoring.
In real-world studies, a subject (e.g. a patient in medical research) can be dropped out for various reasons before an event of interest (e.g. death) happens, which prevents investigators from fully following up \cite{leung1997censoring}.
% censored data는 이러이러해서 어렵다 라는 한줄 들어가면 연결이 좀 더 부드러울 듯.
The presence of censoring in survival data can create a serious challenge in applying standard statistical learning strategies. 
Usually, the censoring process is assumed to be non-informative in that it is irrelevant of the underlying failure process given features, but their relationship should be properly accounted for, otherwise leading to biased results. 


% Main approaches (Cox, AFT) and limitations of each
% Standard Cox
% partial likelihood estimation이라서 large dataset 학습 어려움.
The most popular and standard approach for modeling time-to-event data is Cox's proportional hazards (CoxPH) model.
% The CoxPH relates a conditional hazard to given covariates by multiplicative forms of baseline hazard and exponential covariate effects, and it can be understood by relative risk for the binary covariate.
CoxPH relates a conditional hazard to given features in a  multiplicative form between the baseline hazard function and exponentiated regression component consequently to learn relative risks.
% It is not required to specify a time-dependent baseline hazard function in a parametric form, modeled by nonparametric manner.
% Cox 모델 특징 소개: order 
% Cox 모델 장점 : Cox PH model is “robust”: Will closely approximate correct parametric model 그래서 정확한 form 모르면 괜찮은 초이스가 될 수 있음 -> 얘는 오히려 AFT의 단점을 부각할때 얹어도 될듯./  baseline hazard is not specified (kleinbaum2010survival 122 페이지)
It often works on the assumptions of  proportional hazards and time-invariant covariate-effects, which are difficult to follow in many applications \cite{aalen1994effects}. 
Statistical testing procedures, such as  Schoenfeld's test, are usually conducted to examine these underlying assumptions since many Cox-based analyses are vulnerable to violation of model assumptions. \cite{aalen2001understanding,kleinbaum2010survival}.


% The variants of the Cox model have been developed corresponding to types of regularizers such as Ridge, Lasso, EN, and OSCAR \cite{verweij1994penalized,tibshirani1997lasso,simon2011regularization,vinzamuri2013cox}.
% CoxPH violation 취약: 
% Time distribution 예측 어려움->DATE 논문에 레퍼런스 있음.


% Standard AFT
% maximum likelihood estimation이라서 SGD랑도 잘맞음 
On the other hand, the accelerated failure time model (AFT) or accelerated life model relates the logarithm of the failure time to the features in a linear fashion \cite{lee2003statistical}.  
As a result of its natural physical interpretation and the connection with linear models, this model has served as an attractive alternative to the CoxPH for the regression analysis of censored failure time data.
%On the other hand, once direct modeling on event time is required, AFT model has been a great %alternative to the hazard-based models.
%in that it can estimate survival time distribution while CoxPH focuses on the estimation of covariate effects \cite{aalen1994effects}.
Unlike CoxPH, standard AFT model often parametrizes the underlying time-to-event distribution up to a set of finite-dimensional parameters by using, for example,  Weibull and log-normal distributions. 
%Recently, AFT models have also been explored in deep-learning literature, but not many, mostly parametrizing the underlying residual distribution up to a set of finite-dimensional parameters such as Weibull and log-normal \cite{lee2003statistical}.
% DATE: accelerate / delay assumption 이 clinical에 잘 맞는다. AFT assumes the effect of the covariates accelerates or delays the life course, which is often meaningful in a clinical or pharmaceutical setting, and sometimes ...
% DATE: Learning in AFT models falls into the category of maximum likelihood estimation, and therefore it scales well to large datasets, when trained via stochastic gradient descent. Further, AFT is also more robust to unobserved variation effects, relative to Cox-PH (Keiding et al., 1997).
However, imposing distributional assumption is too strict in real data analysis and can reduce the attractiveness inherent in the AFT model, mostly underperforming Cox-based analysis \cite{cox2008generalized,kleinbaum2010survival}.
% In this work, we explore a rank-based semiparametric estimation of the AFT model, where the residual distribution is completely unknown and thus can be flexibly adapted to given datasets. 
Recently, based on statistical theories and the advent of deep learning techniques, various time-to-event models have been explored to circumvent the necessity of assumptions such as linearity, single risk, discrete time, and fixed-time effect
\cite{katzman2018deepsurv,lee2018deephit,ren2019deep,kvamme2019continuous,avati2020countdown,tarkhan2021survival,rahman2021deeppseudo}.
%time-independency, linearity, competing risk?

% Because of the differences in properties of Cox and AFT, researchers have selected an appropriate tool according to the intention.
% emerging techniques (DATE, CoxTime) 장단점
% 단점 - Heavy
% DNN으로 assumption 깬 논문들 (단순히 딥러닝 적용뿐 아니라, assumption 깨야함)

For example, \textit{Cox-Time} \cite{kvamme2019time} and 
\textit{DATE} \cite{chapfuwa2018adversarial}
alleviate the most fundamental but strict assumptions of the CoxPH and parametric AFT models by allowing non-proportional hazards and non-parametric event-time distribution, respectively.
% PH assumption과 time distribution assumption이 각각 CoxPH, AFT의 '가장' 큰(fundamental) assumption이라는 레퍼런스 찾아보기
% CoxTime
\textit{Cox-Time} exploits neural networks as a relative risk model to access interactions between time and features.
The authors also show that their loss function is a good approximation for the Cox partial log-likelihood.
% DATE
\textit{DATE} is a conditional generative adversarial network that implicitly specifies a time-to-event distribution within the AFT model framework.
It does not require a pre-specified distribution in the form of a parameter, instead the generator can learn from the data using an adversarial loss function.
Incidentally, various deep learning-based approaches have been spotlighted to improve their performance by resolving issues such as temporal dynamics and model calibration \cite{lee2019dynamic,nagpal2021dcm,gao2021multi,kamran2021estimating,hu2021transformer}.
Therefore, it became important to utilize well-designed objective functions that fit not only statistical properties but also optimization of neural networks.
% Incidentally, assumption 해결은 아니지만 딥러닝 기술 적용해서 issue (such as overfitting, temporal dynamics, calibration, )해결한 Survival 논문들 한줄소개. \cite{lee2019dynamic,nagpal2021dcm,kim2020improved,gao2021multi,kamran2021estimating,hu2021transformer} -> 뉴럴넷에 적합한 loss function을 잘 정의하는 것의 중요성이랑도 이어질 수 있음.

% In the lighten of the foregoing findings, there has not been yet sufficiently studied on AFT-based neural networks, contrary to the abundant hazard-based models.
In this paper, we introduce a Deep AFT Rank-regression for Time-to-event prediction model (\textit{DART}), a deep learning-based semiparametric AFT model, trained with an objective function originated from Gehan's rank statistic. % AFT model 연구 잘 없다는 점 언급.
This model eliminates the need to specify a baseline event time distribution, while retaining the benefits of standard AFT models that directly predict event times.
By constructing comparable rank pairs in the simple form of loss functions, the optimization of \textit{DART} is efficient compared to other deep learning-based event time models.
Our numerical experiments show that \textit{DART} not only calibrates well, but also competes in its ability to predict the sequence of events compared to risk-based models.
% (use-scenario 안 쓸 거면 일단 주석처리) We also provide use scenarios for the interpretation of marginal covariate impacts.
% With regard to abundant studies for hazard-based models, deep learning-based AFT studies are left relatively unexplored. 
% We believe that this work can be widely applied in the community while giving prominence to advantages of the AFT model.
Furthermore, we believe that this work can be widely applied in the community while giving prominence to advantages of the AFT model that is relatively unexplored.%, with regard to abundant studies for hazard-based models.

%We believe that this work can contribute to the community while giving prominence to advantages of the AFT model.
% Our contribution
% 1. Rank loss 의 장점 with theoretical background. without loss of advantages of standard AFT model.
% 2. Simple & Fast to optimize
% 3. Better performance indicating well-calibrated
% log-rank statistic은 survival function을 estimation하는 statistic -> reference 필요.
% Transformer, RNN, CNN 등을 사용한 최신 연구들과도 조합이 잘 됨.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Introduction}
% Importance of data-driven decision making is inarguable in various industries such as manufacturing, retail as well as biomedical research field. Personalized or precision medicine becomes more  promising in medical application of machine learning, which utilizes patients' information to customize treatment option for maximal response. To do so, it is crucial to predict expected recuperation rate or life expectancy of target treatment option using patients' demographic features and previous medical records.
% Survival analysis is the main tool when research interest lies on expected hazard of event occurrence or expected time-to-event to given covariate information. Based on statistical theories and advent of modern machine learning methods, many survival models have been explored, especially with utilizing deep neural networks (DNN), 
% to find  prominent results in prediction. 

% However, there are many unresolved topics for survival neural networks. One is the necessity of generalization in terms of both theory and empirical performance. Although deep learning techniques have shown dominant predictive power, they still require stringent assumptions, such as proportionality of hazards, pre-determined probability distribution, etc. Another issue with survival regressions based on machine learning or neural network is explainability upon outcome.
% High predictability and model flexibility in these approaches are obtained at the expense of 
% direct interpretation that is critical in medical application. 
% In addition, most deep learning algorithms were often designed within the Cox proportional hazards framework, in which hazard ratio is usually the target response, 
% but is hard to interpret when combined with neural networks.

% Through these points, we propose a generalized version of survival regression model, both theoretically and empirically, without much loss of predictive performance and interpretability.  We also prove the utility of the proposed method, by 
% applying it to optimal treatment allocation problem for precision medicine.
% Our implementation is publicly available at: \url{https://github.com/DART-submission/anonymous}

==> sections/2_related_work_old.tex <==
\section{Related Works}

We first overview time-to-event modeling focusing on the loss functions of \textit{Cox-Time} and \textit{DATE} models to highlight the difference in concepts before introducing our method.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               2.1 Preliminaries
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Preliminaries}
The primary interest of time-to-event analysis is to estimate survival quantities like survival function $S(t)=P(T \ge t)$ or hazard function $h(t)=\lim_{\delta \rightarrow 0}P(t \le T \le t + \delta|T \ge t)/\delta $, where $T \in \mathbb{R}^+$ denotes time-to-event random variable. 
In most cases, due to censored observations, those quantities cannot be directly estimated with standard statistical inference procedure. 
In the presence of right censoring, \citet{kaplan1958nonparametric} and \citet{aalen1978nonparametric} provided consistent nonparametric survival function estimators, exploiting right-censoring time random variable $C \in \mathbb{R}^+$. 
% Researchers then can get stable estimates for survival quantities with  data tuples $\{(y_i, \delta_i,X_i),i=1,...,N\}$, where $y_i = \min (T_i, C_i)$ is observed event time with censoring, $\delta_i = I(T_i \le C_i)$ is censoring indicator, and covariate  $X \in \mathbb{R}^{N \times P}$. 
Researchers then can get stable estimates for survival quantities with  data tuples $\{y_i, \delta_i,X_i\}_{i=1}^N$, where $y_i = \min (T_i, C_i)$ is the observed event time with censoring, $\delta_i = I(T_i \le C_i)$ is the censoring indicator, and a vector of features  $X_i \in \mathbb{R}^{P}$. 
Here, $N$ and $P$ denote the number of instances and  the number of features, respectively. 
While those nonparametric methods are useful, one can  improve predictive power by incorporating feature information in a way of regression modeling. 
Cox proportional-hazards (CoxPH) and accelerated-failure-time (AFT) frameworks are the most common approaches in modeling survival quantities utilizing both censoring and features.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               2.2 Non-linear CoxPH models
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Hazard-Based Models}

A standard CoxPH regression model \cite{cox1972regression} formulates 
the conditional hazard function as:
\begin{equation}
h(t|X_i)=h_0(t)\exp(\beta^T X_i),~(i=1,\ldots,N),
\end{equation}
where $h_0(\cdot)$ is an unknown baseline hazard function which has to be estimated nonparametrically, and $\beta \in \mathbb{R}^{P}$ is the regression coefficient vector. 
It is one of the most celebrated models in statistics in that $\beta$ can be estimated at full statistical efficiency while achieving nonparametric flexibility on $h_0$ under the proportionality assumption. 
Note the model is semiparametric due to the unspecified underlying baseline hazard function $h_0$.
%probability distribution of random variable $T_i$.
%
Letting $\mathcal{R}_i$ be the set of all individuals ``at risk'', meaning that are not censored and have not experienced the event before $T_i$, statistically efficient estimator for regression coefficients can be obtained minimizing the loss function with respect to $\beta$:
\begin{equation}\label{cox}
L_{\text{CoxPH}}(\beta) = \sum_{i}\delta_i\log\left( \sum_{j\in \mathcal{R}_i}  \exp\left[\beta^T X_j - \beta^T X_i\right] \right),
\end{equation}
which is equivalent to the negative partial log-likelihood function of CoxPH model.

Based on this loss function, \citet{kvamme2019time} proposed a deep-learning algorithm for the hazard-based predictive model, namely \textit{Cox-Time}, replacing $\beta^TX_j$ and $\beta^TX_i$ with $g(y_j, X_j; \theta)$ and $g(y_i, X_i; \theta)$, respectively. % to alleviate the proportionality of hazards and the linearity assumption between response and covariates.
% \begin{equation}
% L_{\text{CoxTime}}(\theta) = \sum_{i}\delta_i\log\left( \sum_{j\in \mathcal{\tilde{R}}_i}  \exp\left[g(y_i, X_j; \theta) - g(y_i, X_i; \theta)\right] \right)
% \end{equation}
Here, $g(\cdot)$ denotes the neural networks parameterized by $\theta$, and $\mathcal{R}_i$ would be replaced by $\tilde{\mathcal{R}}_i$, representing the sampled subset of $\mathcal{R}_i$. 
With a simple modification of the standard loss function in Eq. (\ref{cox}), \textit{Cox-Time} can alleviate the proportionality for relative risk,
showing empirically remarkable performance against other hazard-based models in both event ordering and survival calibration.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               2.3 Parametric AFT models
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Accelerated-Failure-Time Models}

The conventional AFT model relates the log-transformed survival time to a set of features in a linear form:
\begin{equation} \label{aft_model}
\log T_i  = \beta^T X_i + \epsilon_i,~(i=1,\ldots,N),
\end{equation}
where $\epsilon_i$ is an independent and identically distributed error term with a common distribution function $F_0(\cdot)$ that is often assumed to be  Weibull, exponential, log-normal, etc.
As implied in Eq. (\ref{aft_model}), AFT model takes a form of linear modeling and provides an intuitive and physical interpretation on event time without detouring via the vague concept of hazard function, making it a powerful alternative to hazard-based analysis. 
However, imposing a parametric distributional assumption for $\epsilon_i$ is a critical drawback of the model, for which model in Eq. (\ref{aft_model}) could be a subclass of the hazard-based models. 

To alleviate linearity and parametric distributional assumptions, several works brought the concept of generative process and approximated the error distribution via neural networks like generative adversarial network (GAN) \cite{miscouridou2018deep,chapfuwa2018adversarial}. 
Especially, \citet{chapfuwa2018adversarial} proposed a deep adversarial time-to-event (\textit{DATE}) model, which specifies the loss function as:
% \begin{equation}
%     L_{\text{DATE}}(\theta, \phi) = L_1(y_i, X_i; \theta, \phi, \delta_i = 1) + \lambda_2 L_2(y_i, X_i; \theta, \delta = 0) + \lambda_3 L_3 (y_i, X_i; \theta, \delta = 1)
% \end{equation}
\begin{align}
\label{DATE}
    L_{\text{DATE}}(\theta, \phi) &=  \mathbb{E}_{(X, y) \sim F_{nc}}[D_\phi(X, y)]   \\
    +& \mathbb{E}_{X\sim F_{nc}, \xi\sim F_{\xi}}[1 - D_\phi(X, G_\theta(X, \xi; \delta = 1))] \nonumber \\ 
    +& \lambda_2 \mathbb{E}_{(X, y)\sim F_{c}, \xi \sim F_{\xi}}[\max(0, y - G_\theta(X, \xi; \delta = 0))] \nonumber \\
    +& \lambda_3 \mathbb{E}_{(X, y) \sim F_{nc},\xi \sim F_{\xi}}[\| t - G_\theta(X, \xi; \delta = 1) \|_1] \nonumber
\end{align}
where $\theta$ and $\phi$ denote the parameter set 
associated with a generator $G_\theta$ and a discriminator $D_\phi$, respectively,
$(\lambda_2, \lambda_3)$ are hyperparameters to tune censoring trade-off, 
$F_{nc}(X, y)$ and  $F_{c}(X, y)$ are empirical joint distributions for non-censored cases and censored cases, respectively, and $F_{\xi}$ is the simple distribution, such as uniform distribution.
The generator $G_\theta$ implicitly defines event time distribution.
Despite \textit{DATE} achieves prominent survival calibration via the sample-generating process, the objective function is quite complicated and the GAN framework is inherently prone to mode collapse, i.e., the generator learns only a few modes of the true distribution while missing other modes \cite{srivastava2017veegan}.
Also, when optimizing neural networks with multiple loss functions, it is difficult to balance and there might be conflicts (i.e. trade-off) with each term \cite{Dosovitskiy2020You}.
Therefore, their loss function might be difficult to be optimized as intended and requires a burdening training time, and consequently not be suitable for large-scale time-to-event analysis.
%Considering the complexity of the loss function and GAN architecture to handle time-to-event distribution, it might not be suitable for large-scaled time-to-event analysis.
% \begin{align*}
%     L_1 &= \mathbb{E}_{(y, X) \sim F_{nc}}[D(X, y)] + \mathbb{E}_{X\sim F_{nc}, \xi\sim F_{\xi}}[1 - D(X, G(X, \xi; \theta, \delta = 1))] \\
%     L_2 &= \mathbb{E}_{(y, X)\sim F_{c}, \xi \sim F_{\xi}}[\max(0, y - G(X, \xi; \theta, \delta = 0))]\\
%     L_3 &= \mathbb{E}_{(y, X) \sim F_{nc}}[|| t - G(X, \xi; \theta, \delta = 1) ||_1]
% \end{align*}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the statistical literature, there have been many attempts to directly estimate regression coefficients in the semiparametric AFT model, where  the error distribution $F_0$ is left unknown, rather than imposing specific parametric distribution or  exploiting generative models. 
In this work, we bridge non-linear representation learning and an objective function for estimation of semiparametric AFT model, which is originated from Gehan's rank statistic.
%In this work, we adopt a rank-based loss function for the semiparametric AFT, originated from Gehan's rank statistic, which is simple but theoretically fundamental.
%We and extend it to a more generalized version throughout neural networks. 
By extensive quantitative analysis, we have shown the beauty of simplicity and compatibility of rank-based estimation, along with outstanding experimental performance.

==> sections/5_experiments_old.tex <==
\section{Experiments}




% \begin{table}[t]
% \caption{Summary of WDSM KKBox customer churn prediction dataset}
% \label{table_2}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lrrr}
% \toprule
% Dataset & Size & \# Unique & \% Censored \\
% \midrule
% Train      & 1,786,333 & 1,582,202 & 0.28 \\
% Test       & 661,748   & 586,001   & 0.28 \\
% Validation & 198,665   & 175,801   & 0.28 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}



In this section, we describe our experiment design and results to validate performance of \textit{DART} compared to other time-to-event regression models. 
Experiments are done with four real-world survival datasets, and baseline models provided by \citeauthor{kvamme2019time} and \citeauthor{chapfuwa2018adversarial}, using two evaluation metrics mentioned in previous section. 
% Model architecture and optimization details are also summarized.



%\begin{table*}[t]
%\label{table_4}
%\caption{Mean and standard deviation of Integrated Negative Log-likelihood (IBLL)}
% \vskip 0.15in
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{lcccc}
%\toprule
%Model & WSDM KKBox & GBSG & FLCHAIN & SUPPORT  \\
%\midrule
%\textit{DeepSurv} & --0.349 (0.001) & --0.517	(0.007) & \underline{--0.332}	(0.019) & %\underline{--0.560}	(0.011)  \\
%\textit{DeepHit}  & --0.402 (0.003) & --0.550	(0.052) &--0.628	(0.466)&  --0.643	(0.095) \\
%%\textit{Cox-CC}   & --0.376 (0.074) & --0.526	(0.010) & --0.574	(0.454) & --0.562	(0.007)  \\
%\textit{Cox-Time} & \underline{--0.338} (0.071) & \underline{--0.516}	(0.011) & --0.400	(0.087) & %--0.571	(0.015)  \\
%\textit{DRAFT} & - & - & - & - \\
%\textit{DATE} & - & - & - & - \\
%\textit{DART (ours)}    & \textbf{--0.321} (0.003) &\textbf{--0.438}	(0.064) &\textbf{--0.232}	%(0.022) & \textbf{--0.531}	(0.024)\\
%\bottomrule
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\vskip -0.1in
%\end{table*}


\begin{table*}[h]
\caption{Summary of survival datasets.}
\label{table_1}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lrrr}
\toprule
Dataset & Size & \# features & \% Censored \\
\midrule
WSDM KKBox     &2,646,746 & 15  & 0.28\\
SUPPORT      & 8,873 & 14 & 0.32 \\
FLCHAIN      & 6,524 & 8  & 0.70 \\
GBSG & 2,232 & 7  & 0.43 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               5.1 datasets
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Datasets}
We choose three common survival datasets and a single large-scale dataset provided by \citeauthor{kvamme2019time}.
The descriptive statistics are provided in Table \ref{table_1}.
First, three common survival datasets that used in this work are the Study to Understand Prognoses Preferences Outcomes and Risks of Treatment (SUPPORT), the Assay of Serum Free Light Chain (FLCHAIN), and the Rotterdam tumor bank and German Breast Cancer Study Group (GBSG). 
% Especially, GBSG contains indicator variable for hormonal therapy, which can be applied to verify effectiveness of treatment recommender system built with survival regression models.
In addition, WSDM KKBox from preparation for the 11th ACM International Conference on Web Search and Data Mining is the dataset for customer churn prediction containing millions of instances and 15 covariate variables. 
With this large-scale dataset, consistency of training procedure and predictive performance would clearly be verified.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               5.2. Baseline Models
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Baseline Models}
We select six neural network-based time-to-event regression models as our experimental baselines: \textit{DRAFT} and \textit{DATE} \cite{chapfuwa2018adversarial} as AFT-based models for direct comparison with our model, and \textit{DeepSurv} \cite{katzman2018deepsurv},  \textit{Cox-CC} and \textit{Cox-Time} \cite{kvamme2019time} as hazard-based models.
%, \textit{DeepHit} \cite{lee2018deephit} as a PMF-based model for references. 

For AFT-based models, \textit{DRAFT} utilizes neural networks to fit log-normal parametric AFT model in non-linear manner. 
That is, it might be misspecified if true error variable does not follow log-normal distribution. 
In contrast, \textit{DATE} exploits generative-adversarial networks (GANs) to learn conditional time-to-event distribution and censoring distribution using observed dataset. 
% Although the approach is not purely nonparametric as authors had mentioned, parametric-distributional assumptions has been alleviated via generative model deriving improved performance against AFT-based models with pre-specified parametric distribution.

In case of hazard-based models, \textit{DeepSurv} fits Cox regression model whose output is estimated from neural networks. 
The model outperforms the standard CoxPH model in performance, not clearly exceeding other neural network-based models.
Furthermore, the proportional hazards assumption still remains unsolved with \textit{DeepSurv}.
\textit{Cox-CC} is another neural network-based Cox regression model, using case-control sampling for efficient estimation. 
While both \textit{DeepSurv} and \textit{Cox-CC} are bounded to proportionality of baseline hazards, \textit{Cox-Time} relieves this restriction using event-time variable to estimate conditional hazard function.
%By doing so, \textit{Cox-Time} has turned out to be superior for survival calibration in many cases.

% In addition, we include \textit{DeepHit} \cite{lee2018deephit} as a reference, which is a survival regression model parameterizing discrete-time hazard rate with neural networks based on survival probability mass function (PMF), considering its contribution to alleviate the fundamental assumption of hazard-based and AFT-based models.
% Although its prediction performance has been reported prominent to others, the training procedure is quite unstable which is a critical shortcoming for practical application. 


Except for neural network-based models, we exclude other machine learning-based models from baselines regarding comparison from previous studies. 
% since they have been verified to be superior to others in terms of both prediction and survival calibration through previous studies.
Some neural network-based models are excluded as well in this study since we focus on alleviating fundamental assumptions such as proportionality and parametric distribution.
% Some neural network-based models has been excluded in this studies since we focus on 
Note that comparing hazard-based models and AFT-based models has rarely been studied due to their difference in concepts: modeling hazard function and modeling time-to-event variable. 
Despite models can be evaluated with common metrics, analysis upon numerical experiments has to be cautious, especially between a hazard-based model and an AFT-based model. 



\begin{table*}
    % \scriptsize
% \caption{Mean and standard deviation of $C^{\text{td}}$. The \textbf{boldface} and  the \underline{underline} denote best and second best performance.}
\caption{Mean and standard deviation of $C^{\text{td}}$. 
% The \textbf{boldface} denotes best performance.
% PMF denotes a method parameterizing the probability mass function.
HAZ and AFT denote hazard-based and AFT-based methods, repectively.}
\label{table_2}
% \vskip 0.15in
% \captionsetup{justification=centering}
% \vskip -0.6in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{clcccc}
\toprule
\multicolumn{2}{c}{MODEL}  & WSDM KKBox  & SUPPORT & FLCHAIN& GBSG  \\
\midrule
% PMF&\textit{DeepHit}  &0.553 (0.002) & 0.645	(0.009)  &0.797(0.015) & 0.684 (0.013)\\
% \midrule
\multirow{3}{*}{\rotatebox{90}{HAZ}}&\textit{DeepSurv} &0.841 (0.000)  & 0.619	(0.008)  & 0.797	(0.013)& 0.685 (0.013)\\
&\textit{Cox-CC}   & 0.836 (0.046)& 0.618	(0.009) & 0.797(0.013) & 0.684 (0.012) \\
&\textit{Cox-Time} & \textbf{0.853} (0.049)& \textbf{0.637}	(0.009)   &\textbf{0.800}	(0.012)& \textbf{0.687} (0.012)\\
\midrule
\multirow{3}{*}{\rotatebox{90}{AFT}} &\textit{DRAFT} & 0.861 (0.005)  & 0.599	(0.018)& 0.725	(0.057)& 0.611 (0.016)  \\
&\textit{DATE} & 0.852 (0.001)  & 0.608	(0.008)& 0.784	(0.009) & 0.598 (0.034)  \\
&\textit{DART (ours) }    & \textbf{0.867} (0.001)&  \textbf{0.624}	(0.009) & \textbf{0.797}	(0.014) &\textbf{0.687} (0.014) \\
\bottomrule
\end{tabular}
% \end{sc}
% \end{small}
\end{center}
% \vskip -0.1in
\end{table*}



\begin{table*}[t]
% \captionsetup{justification=centering}
\caption{Mean and standard deviation of Integrated Brier Score (IBS).}
\label{table_3}
    % \scriptsize
% \vskip 0.15in
\begin{center}
% \begin{small}
% \begin{sc}
\begin{tabular}{clcccc}
\toprule
\multicolumn{2}{c}{MODEL}  & WSDM KKBox & SUPPORT & FLCHAIN &  GBSG \\
\midrule
% PMF & \textit{DeepHit}  &  0.124 (0.001)&0.221	(0.034)  & 0.160	(0.081) & 0.183	(0.015)\\
% \midrule
\multirow{3}{*}{\rotatebox{90}{HAZ}}&\textit{DeepSurv} &0.111 (0.000) &  \textbf{0.190}	(0.004) & \textbf{0.101}	(0.006) & \textbf{0.174}	(0.004)\\
&\textit{Cox-CC}   & 0.115 (0.012) &  0.191	(0.003) & 0.122	(0.028) &0.177	(0.004) \\
&\textit{Cox-Time} & \textbf{0.107} (0.009) & 0.194	(0.006) & 0.114	(0.016) & \textbf{0.174}	(0.005) \\
\midrule
\multirow{3}{*}{\rotatebox{90}{AFT}} &\textit{DRAFT} & 0.147 (0.002) & 0.314	(0.043) &0.144	(0.022) & 0.310	(0.010) \\
&\textit{DATE} & 0.131 (0.002) & 0.227	(0.004) & 0.124	(0.012) & 0.204	(0.004) \\
&\textit{DART (ours) } &\textbf{0.108} (0.001) &\textbf{0.176}	(0.005)  &  \textbf{0.068}	(0.007)&  \textbf{0.150}	(0.023) \\
\bottomrule
\end{tabular}
% \end{sc}
% \end{small}
\end{center}
\vskip -0.1in
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               5.3. Architecture and Optimization
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Model Specification and Optimization Procedure}
For a fair comparison, we apply neural network architecture used in \citeauthor{kvamme2019time}: MLP with dropout and batch-normalization. 
Every dense blocks are set to have the equal number of nodes, no output bias is utilized for output layer, and ReLU function is chosen for non-linear activation for all layers.
Preprocessing procedure has also been set based on \citeauthor{kvamme2019time} including standardization of numerical features, entity embeddings \cite{guo2016entity} for multi-categorical features. 
The dimension of entity embeddings is set to half size of the number of categories.
In addition, due to the fact that parameters of AFT-based models tend to be influenced by scale and location of the target variable, $y$ has been standardized and its mean and variance are separately stored to rescaled outputs. 
% For SGD algorithm, AdamWR \cite{loshchilov2017decoupled} is used as implemented by \citeauthor{kvamme2019time} with one epoch of an initial cycle length.
% We also set the cycle length to double after each cycle.
% The details about data split and hyperparameter search are described in the appendix.

% WSDM KKBox contains the fixed train/valid/test split, so we perform grid search for hyperparameters and repeat the same experiments with the best configuration and different random seeds.
% For the other three datasets, we perform 5-fold cross-validation because they are relatively small and not containing fixed data splits.
% The best hyperparameter sets are determined among 300 random configurations for each fold.
% The details of the experimental setting are described in the appendix.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               5.4. Experimental Settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Experimental Settings}


% \begin{table*}[t]
% \caption{Hyperparameter search space for GBSG, FLCHAIN, and SUPPORT datasets.}
% \label{tab:hyper_others}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{tabular}{lccc}
% \toprule
% Hyperparameter &Values \\
% \midrule
% \# Layers &\{1, 2, 4\} \\
% \# Nodes per layer & \{64, 128, 256, 512\}   \\
% Dropout & \{0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7\} \\
% Weight decay & \{0.4, 0.2, 0.1, 0.05, 0.02, 0.01, 0.001\}\\
% Batch size & \{64, 128, 256, 512, 1024\}\\
% % $\alpha$ (DeepHit) & \{0.0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1.0\} \\
% % $\sigma$ (DeepHit) & \{0.1, 0.25, 0.5, 1, 2.5, 5, 10, 100\} \\
% % Num. durations (DeepHit) & \{50, 100, 200, 400\} \\
% $\lambda$ (CoxTime and CoxCC) & \{0.1, 0.01, 0.001, 0.0\} \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

% \begin{table}[t]
% \caption{Hyperparameter search space for the WSDM KKBox dataset.}
% \label{tab:hyper_kkbox}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{tabular}{lccc}
% \toprule
% Hyperparameter &Values \\
% \midrule
% \# Layers &\{4,6,8\} \\
% \# Nodes per layer & \{128, 256, 512\}   \\
% Dropout & \{0.0, 0.1, 0.5\} \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


% \begin{table}[t]
% \caption{Best configurations for WSDM KKBox dataset.}
% \label{tab:hyper_kkbox_best}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{tabular}{lccc}
% \toprule
%  MODEL & \# Layers & \# Nodes & Dropout  \\
% \midrule
% % \textit{DeepHit} &6 &512 &0.1  \\
% \textit{DeepSurv} &6 & 256& 0.1 \\
% \textit{Cox-CC} & 6& 128& 0.0 \\
% \textit{Cox-Time} & 8& 256& 0.0 \\
% \textit{DRAFT}  & 8& 128& 0.0 \\
% \textit{DATE} & 8& 512& 0.5 \\
% \textit{DART (ours)} & 6& 256& 0.0 \\
% \bottomrule 
% \end{tabular}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}


\textbf{\textit{DeepSurv, Cox-CC, Cox-Time, DART}.} 
The PyCox\footnote{https://github.com/havakv/pycox} python package provides the training codes for these models.
For WSDM KKBox dataset, we repeat experiments 30 times with best configurations provided by \citeauthor{kvamme2019time}.
Because train/valid/test split of KKBox dataset is fixed, we don't perform a redundant search procedure.
For the other datasets (SUPPORT, FLCHAIN, and GBSG), we perform 5-fold cross-validation as performed at \citeauthor{kvamme2019time} because the size of datasets is relatively small.
At each fold, the best configuration is selected among 300 combinations of randomly selected hyperparameters which are summarized in Table \ref{tab:hyper_others}.
We use AdamWR \cite{loshchilov2017decoupled} starting with one epoch of an initial cycle and doubling the cycle length after each cycle.
The batch size is set to 1024 and the learning rates are found by \citeauthor{smith2017cyclical} as performed at \citeauthor{kvamme2019time}.



\textbf{\textit{DRAFT, DATE}.} 
The implementation of \textit{DATE}\footnote{https://github.com/paidamoyo/adversarial\_time\_to\_event} by the authors includes the code of \textit{DRAFT} as well.
We utilize their official codes for all datasets.
The batch size for KKBox dataset is set to 8192 because the experiments are not feasible with the batch size 1024 due to their training time.
The best configurations of \textit{DRAFT} and \textit{DATE} also are founded by grid search with same hyperparameter search space with others.
We repeat experiments 30 times with the best configuration as mentioned above.
For the other datasets, as same with other models, we perform 5-fold cross-validation and choose the best configuration among 300 random hyperparameter sets at each fold.
% The early stopping is applied as done in other models equally.

% The hyperparameter search space and best configurations for WSDM KKBox dataset are summarized in Table \ref{tab:hyper_kkbox} and in Table \ref{tab:hyper_kkbox_best}, respectively.
Our implementation for \textit{DART} is publicly available at: \url{https://github.com/dart-submission/dart-submission}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               5.4. Evaluation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Performance Evaluation}
To measure discriminative performance of outputs, we exploit standard C-index \cite{harrell1982evaluating} for AFT-based models while letting hazard-based models to utilize $C^{\text{td}}$ since equivalent evaluation is possible for AFT-based models including \textit{DART} since it outputs a single scalar value to evaluate ranks.
In terms of survival calibration, we implement our own function to obtain IBS based on its definition, due to the fact that evaluation methods of the conditional survival function and IPCW provided by \citeauthor{kvamme2019time} are not compatible with AFT-based models. 
Specifically, we first fit Kaplan-Meier estimator upon standardized training set, and subsequently evaluate conditional survival estimates and IPCW utilizing estimated residuals, following the definition of baseline hazard function of AFT framework rather than to use time-to-event variable directly.
For numerical integration, we follow settings of time grid from \citeauthor{kvamme2019time}, and standardize the grid with mean and standard deviation stored with standardization procedure of training set. 
By doing so, IBS can be compared upon identical timepoints for both hazard-based models and AFT-based models.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%               5.5. Summary of Results
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Summary of Results}

Experiment results are provided in Table \ref{table_2} and \ref{table_3}. 
In summary, \textit{DART} is competitive in both discriminative and calibration performance, especially for large-scale survival datasets. 
Specifically, \textit{DART} yields consistent results for WSDM KKBox dataset compared to other baselines, maintaining competitive performance in terms of $C^{\text{td}}$ and IBS. 
We point out that \textit{DART} is the most powerful and AFT-based time-to-event model that can be a prominent alternative when hazard-based models might be not working.
% Detailed analysis on experiments will be provided in the next section.






==> tables/ablation.tex <==
\begin{table}
\tiny
  %The ground-truth of IMDB-M is calculated by Beam, Hungarian, and VJ. }
  \centering
  \small
  \begin{tabular}{l|ccc|c}
    \textbf{Methods} & \textbf{GNN} & \textbf{Co-att} & \textbf{Pooling} & \textbf{AUROC} \\ \hline \hline
    %\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
    MPNN-Concat & \checkmark & - & - & 0.661 \\
    MHCADDI-ML & \checkmark & \checkmark & - & 0.819 \\ 
    TopKPool & \checkmark & - & \checkmark & 0.847 \\
    SAGPool  & \checkmark & - & \checkmark & 0.862 \\ \hline
    \textbf{Ours} & \checkmark & \checkmark & \checkmark & \textbf{0.891} \\
  \end{tabular}
  \caption{Ablation studies and comparison with other pooling methods on the Decagon test set. Note that the scope of this ablation study only includes methods that do \textbf{not} use additional information such as protein features or one-hot encoding of the interaction.}
  \label{tab:ablation}
\end{table}

==> tables/auprc.tex <==

% \begin{sidewaystable}

% \begin{landscape}
\begin{table}
  %The ground-truth of IMDB-M is calculated by Beam, Hungarian, and VJ. }
  \centering
  \small{
  \begin{tabular}{l|ccc}
    \textbf{Methods} & \textbf{AUROC} & \textbf{AUPRC} & \textbf{AP@50} \\ \hline  \hline
    %\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
    RESCAL & 0.693 & 0.613 & 0.476 \\
    DEDICOM & 0.705 & 0.637 & 0.567 \\
    DeepWalk & 0.761 & 0.737 & 0.658 \\
    Concatenated features & 0.793 & 0.764 & 0.712 \\
    Decagon & 0.872 & 0.832 & 0.803 \\ \hline
    \textbf{Ours} & \textbf{0.891} & \textbf{0.867} & \textbf{0.812} \\
  \end{tabular}}
  \caption{Evaluation results under AUPRC and AP@50 on the Decagon test set for a more precise comparison with baselines that provide their performance under these metrics.}
  \label{tab:eval_table}
\end{table}
% \end{sidewaystable}

==> tables/auroc.tex <==
\begin{table}
  %The ground-truth of IMDB-M is calculated by Beam, Hungarian, and VJ. }
  \centering
  \footnotesize{
  \begin{tabular}{l|c|c}
    \textbf{Methods} & \textbf{feature+} & \textbf{AUROC} \\ \hline \hline
    %\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9}
    Concatenated features & \checkmark & 0.793 \\
    Decagon & \checkmark & 0.872 \\
    Late-Outer & \checkmark & 0.724 \\
    CADDI& \checkmark & 0.778 \\
    MHCADDI & \checkmark & 0.882 \\ \hline 
    MPNN-Concat  & - & 0.661 \\
    Drug-Fingerprints  & - & 0.744 \\
    RESCAL& - & 0.693 \\
    DEDICOM & - & 0.705 \\
    DeepWalk & - & 0.761 \\
    MHCADDI-ML & - & 0.819 \\ \hline
    \textbf{Ours} & - & \textbf{0.891} \\
  \end{tabular}
  }
  \caption{AUROC results on the Decagon test set. The \checkmark under the feature+ column indicates that the according baseline leverages external features other than the drug itself such as protein-protein interaction or the one-hot encoding of the drug-drug interaction (the target class).
%   Performance comparison under other metric summarized in Table \ref{tab:eval_table}.
}
  \label{tab:AUROC}
\end{table}

==> tables/ged_results.tex <==
% \begin{adjustbox}{angle=90}
% \begin{center}

% \rotatebox{90}{
% \vbox{


% \begin{landscape}
\begin{table*}
    % \scriptsize
  %The ground-truth of IMDB-M is calculated by Beam, Hungarian, and VJ. }
  \centering
  \begin{tabular}{l|ccc|ccc|ccc}
    & \multicolumn{3}{c|}{\textbf{AIDS}} & \multicolumn{3}{c|}{\textbf{LINUX}} & \multicolumn{3}{c}{\textbf{IMDB-M}}  \\
    \textbf{Methods}     & MSE & $\rho$ & $\tau$ & MSE & $\rho$ & $\tau$ & MSE & $\rho$ & $\tau$ \\
    \hline \hline
%    Beam & 12.090  & 0.609  & 0.463  & 9.268  & 0.827  & 0.714  & - & - & -\\
%    Hungarian &  25.296 &  0.510 &  0.378 & 29.805 &  0.638 &  0.517  & - & - & -\\
%    VJ &  29.157 &  0.517 &  0.383 & 63.863 &  0.581 &  0.450  &- & - & - \\
%    \midrule
    S-Mean & 3.115  & 0.633 & 0.480 & 16.950  & 0.020 & 0.016 & 3.749  & 0.774 & 0.644     \\
    H-Mean & 3.046  & 0.681 & 0.629 & 6.431  & 0.430 & 0.525 & 5.019  & 0.456 & 0.378     \\
    H-Max & 3.396 & 0.655 & 0.505  & 6.575 &0.879& 0.740 & 6.993& 0.455 &0.354     \\
    Att.Deg. &   3.338 & 0.628 & 0.478 &8.064 &0.742 &0.609 &2.144 &0.828 &0.695 \\
    Att.GC & 1.472&  0.813&  0.653& 3.125&  0.904&  0.781&  3.555 & 0.684 & 0.553\\
    Att.LGC &  1.340 &  0.825 &  0.667 & 2.055 &  0.916 &  0.804 &   1.455 &  0.835 &  0.700 \\
    SimGNN & \textbf{1.189}  & 0.843 & 0.690 & 1.509  & 0.939 & 0.830 & 1.264  & 0.878 & 0.770     \\ \hline
    CAGPool &  2.959 &  \textbf{0.880} &  \textbf{0.717} &\textbf{0.658} &\textbf{0.988} &\textbf{0.922} & \textbf{0.884} &\textbf{0.975} &\textbf{0.874}    \\
  \end{tabular}
  \caption{The experimental results of graph similarity regression task. The evaluation metrics are Mean Square Error (MSE, $10^{-3}$), Spearman’s rank correlation coefficient $\rho$, and Kendall’s rank correlation coefficient $\tau$.} 
  \label{tab:GED_results}
\end{table*}
% \end{center}
% \end{adjustbox}

% \end{landscape}

==> tables/hyper_kkbox.tex <==
\begin{table}
\caption{Hyperparameter search space for the WSDM KKBox dataset.}
\label{tab:hyper_kkbox}
% \vskip 0.15in
\begin{center}
\begin{tabular}{lccc}
\toprule
Hyperparameter &Values \\
\midrule
\# Layers &\{4,6,8\} \\
\# Nodes per layer & \{128, 256, 512\}   \\
Dropout & \{0.0, 0.1, 0.5\} \\
\bottomrule
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}

==> tables/hyper_kkbox_best.tex <==
\begin{table}
\caption{Best configurations for WSDM KKBox dataset.}
\label{tab:hyper_kkbox_best}
% \vskip 0.15in
\begin{center}
\begin{tabular}{lccc}
\toprule
 MODEL & \# Layers & \# Nodes & Dropout  \\
\midrule
% \textit{DeepHit} &6 &512 &0.1  \\
\textit{DeepSurv} &6 & 256& 0.1 \\
\textit{Cox-CC} & 6& 128& 0.0 \\
\textit{Cox-Time} & 8& 256& 0.0 \\
\textit{DRAFT}  & 8& 128& 0.0 \\
\textit{DATE} & 8& 512& 0.5 \\
\textit{DART (ours)} & 6& 256& 0.0 \\
\bottomrule 
\end{tabular}
\end{center}
\vskip -0.1in
\end{table}

==> tables/hyper_others.tex <==

\begin{table}
\caption{Hyperparameter search space for GBSG, FLCHAIN, and SUPPORT datasets.}
\label{tab:hyper_others}
% \vskip 0.15in
\begin{small}
\begin{center}
\begin{tabular}{lccc}
\toprule
Hyperparameter &Values \\
\midrule
\# Layers &\{1, 2, 4\} \\
\# Nodes per layer & \{64, 128, 256, 512\}   \\
Dropout & \{0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7\} \\
Weight decay & \{0.4, 0.2, 0.1, 0.05, 0.02, 0.01, 0.001\}\\
Batch size & \{64, 128, 256, 512, 1024\}\\
% $\alpha$ (DeepHit) & \{0.0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1.0\} \\
% $\sigma$ (DeepHit) & \{0.1, 0.25, 0.5, 1, 2.5, 5, 10, 100\} \\
% Num. durations (DeepHit) & \{50, 100, 200, 400\} \\
$\lambda$ (CoxTime and CoxCC) & \{0.1, 0.01, 0.001, 0.0\} \\
\bottomrule
\end{tabular}
\end{center}
\end{small}
\vskip -0.1in
\end{table}
